Strategic Representation

Humans have come to rely on machines for reducing excessive information to manageable representations. But this reliance can be abused -- strategic machines might craft representations that manipulate their users. How can a user make good choices based on strategic representations? We formalize this as a learning problem, and pursue algorithms for decision-making that are robust to manipulation. In our main setting of interest, the system represents attributes of an item to the user, who then decides whether or not to consume. We model this interaction through the lens of strategic classification (Hardt et al. 2016), reversed: the user, who learns, plays first; and the system, which responds, plays second. The system must respond with representations that reveal `nothing but the truth' but need not reveal the entire truth. Thus, the user faces the problem of learning set functions under strategic subset selection, which presents distinct algorithmic and statistical challenges. Our main result is a learning algorithm that minimizes error despite strategic representations, and our theoretical analysis sheds light on the trade-off between learning effort and susceptibility to manipulation.

==> fullInfo.tex <==
\section{A General Strategic  Representation Game}


\begin{algorithm}[H]
    \SetKwInOut{Output}{Representation dependency graph $G = (V,E)$}
    \SetAlgoNoLine
    \renewcommand{\thealgocf}{}
    \DontPrintSemicolon
%    \SetAlgorithmName{$\textsc{Alg}$}{ }{ }
    \caption{$\textsc{Alg}(\mathcal{I})$}
 \textbf{Output:}    Optimal Choice vector $h$
 \;
 \textbf{Initialize:} $ X^{'} := X  $,   $h(z)= -1$ for all $z \in Z$.
 \;
 \While{$X^{'} \neq \emptyset$}{
Choose $x \in X^{'}$ (arbitrarily)  \;
$G(V^{''}, E^{''}) \gets  \textsc{RepDep}(\mathcal{I},x)$ \;
$ val = val + \textsc{Compute}(G, D,v)$ \; 
$X^{'} \gets  X^{'} \setminus  (V^{''} \cap X) $ \; 
$i \gets i+1$ \;
 } 
 \Return $(val, h)$
\end{algorithm}

\begin{algorithm}[H]
    \SetKwInOut{Input}{$\mathcal{I}$}
    \SetKwInOut{Output}{Representation dependency graph $G = (V,E)$}
    \SetAlgoNoLine
    \renewcommand{\thealgocf}{}
    \DontPrintSemicolon
%    \SetAlgorithmName{$\textsc{Alg}$}{ }{ }
    \caption{$\textsc{RepDep}( x)$}
 \textbf{Output:} Representation dependency graph $G = (V,E)$
 \;
 \textcolor{gray}{  $N(V^{'})$ is    set of neighbors of  set $V^{'}$;  i.e.  $  \{ y  | (x,y) \in \ E \ \text{ for some  } \ x \in V^{'}   \}$ . }\;
 \textbf{Initialize:} 
% Choose $x \in X$ arbitrarily\; 
 $V^{'} = \{x\} \cup Z(x)$ \hspace{20pt}  
 $E^{'} = \{(x,z)| z \in Z(x) \}$\;
 \While{$N(V^{'}) \neq \emptyset$}{
$ V^{'} \gets V^{'} \cup N(V^{'})$ \; 
$E \gets E \cup \{ (x,z): z \in Z(x) \text{ and } (x \in V^{'} \land z \notin V^{'}) \vee (x \notin V^{'} \land z \in V^{'})\} $
 } 
 \Return  $(V,E)$
\end{algorithm}

\begin{observation}
$N(x) = Z(x)$ and $N(z) =X(z) $ for all $x \in X$ and $z \in Z$.
\end{observation}
\begin{figure}[ht!]
\begin{minipage}{0.5 \textwidth}
    \centering
    \includegraphics[scale=0.5]{RepDep.png}    
\end{minipage}
\hfill 
\begin{minipage}{0.45 \textwidth}
        \centering
    \includegraphics[scale=0.35]{Example2.png}    
\end{minipage}

    \caption{L: Representation graph for Example 1 R: Representation graph showing Obervation 1 and Observation 2}
    \label{fig:my_label}
\end{figure}
%Notice that the expected payoff to the User is given as $ \sum_{x \in X} \sum_{z \in N(x)} \mathbbm{1}(\phi(x) = z)\cdot p_{x} v(x)$. 
\begin{observation}
Given $x \in X$, if $h(z) = +1$ for any $z \in N(x)$ then the expected payoff to User from $x$ is $p_x \cdot v(x)$.  
\end{observation}
\begin{proof}
Note that $\phi(x)$ maximizes $h$; hence if there is any $z \in N(x)$ then $\phi(x) = z$ is a best response of the System. We have 
$ \sum_{z\in N(x) | h(z) = 1} \mathbbm{1}(\phi(x) = z) p_x \cdot v(x) \cdot  1 = p_x \cdot v(x). $
\end{proof}
Similarly, we have following observation when all the representations are labelled negatively.   
\begin{observation}
Given $x \in X$, if $h(z) = -1$ for all $ z \in N(x)$ then the expected payoff to the User from $x$ is $ - p_x \cdot v(x)$.
\end{observation}
 \begin{algorithm}
 [H]
%    \SetKwInOut{Input}{$\mathcal{I}$}
    \SetKwInOut{Output}{Representation dependency graph $G = (V,E)$}
    \SetAlgoNoLine
    \renewcommand{\thealgocf}{}
    \DontPrintSemicolon
%    \SetAlgorithmName{}{ }{ }
    \caption{$\textsc{Compute}(G,D,v)$}
    Let $G = (V,E)$\;
\uIf{$|V| \leq 1$}{
    \Return 0 \;
  }
  \uElseIf{$|V| =2$}{
$  x := V \cap X$\; 
$z := V \cap Z  $ \;
$h(z) \gets v(x) $ \;
    \Return $p_x$ \;
  }
  \Else{
Select an arbitrary $ z \in V \cap Z$\; 
Let $\mathcal{G}$ := Collection of graphs obtained by removing  $z$ and $N(z)$ and all the edges connecting these vertices.  %\Big \{ G(V^{'},E^{'}) \Big | V^{'} \subseteq V \setminus \{z\} \cup N(z) , E^{'}  \subseteq  E \setminus \{(x,z): x \in N(z)  \}    \Big \}$ \ and \ \ 
\;
$\mathcal{G}^{'} = $ Collection of graphs obtained by removing $z$ and $\{x \in N(z)|N(x)\setminus \{z\} = \emptyset \}$; i.e. all those items for which $z$ is the only representation in $G$.  %\Big \{ G(V^{'},E^{'}) \Big | V^{'} \subseteq V \setminus \{z\} \cup N(z) , E^{'}  \subseteq  E \setminus \{(x,z): x \in N(z)  \}    \Big \}$ \;
\;
Let $(A) = \sum\limits_{x \in N(z)}  p_x \cdot v(x)) + \sum \limits_{G \in %\{ G \setminus  \{z\} \cup N(z)\}
\mathcal{G}} \textsc{Compute}(G,D,v) $ \ \ and, \; 
\hspace{15pt} $(B) = - \sum \limits_{x \in N(z)| N(x) \setminus \{z\} = \emptyset}  p_x \cdot v(x) + 
\sum \limits_{G \in   
\mathcal{G}^{'}}  
\textsc{Compute}(G,D,v)$\;
$h(z) = \begin{cases}  1 &\text{ if } A \geq  B \\ -1 &\text{Otherwise}  \end{cases}$\;
    \Return \Big( $\max \Big \{ (A) , (B)  \Big \}$ \Big) \; 
  }
  
  \end{algorithm}
  

\begin{theorem}[Proof of Optimality]
\textsc{Alg} finds an User optimal choice function.
\end{theorem}
\iffalse 
\begin{proof}
Consider a representation instance $\mathcal{I}$  with a single representation graph $G = (V,E)$ and let $h^{\star}$ be an optimal User choice function. We prove the theorem  using induction on the number of items i.e. $|X|$.  

\noindent \textbf{Base case}
\underline{$|X|=1$}: 
We have following two cases:

\noindent 1) 
\textbf{$|N(x)| =  1$:} In this case algorithm returns in Line 7 with $h(z) = v(x)$ which is unique optimal solution. 

\noindent 2) \textbf{$|N(x)| >  1$:} In this case algorithm finds an optimal solution with $(A) = p_x v(x) > (B) = 0 $ and returns in Line  16.
\end{proof}
\fi 

\iffalse 
\begin{theorem}
There does not exist and algorithm that  finds an User optimal choice function in sublinear time.
\end{theorem}
\fi 
%\begin{proof}
%Let $\textsc{Opt}(\mathcal{I})$ be the optimal payoff to the user.  
%\begin{lemma}
%Let $G_{1}, G_2, \cdots, G_k $ be representation dependency  graphs created in line 5 of \textsc{Alg} then  $\textsc{Opt}(\mathcal{I}) = \sum_{i } \textsc{Opt}(G_i) $.
%\end{lemma}
%\end{proof}


%Recall,  $Z = \{ \pp \pp, \rr \rr \}$ and $X = \{ \pp, \rr, \{\pp,\rr\} \}$. 
The representation dependency graph for this instance is given in Figure \ref{fig:my_label} (L). It is easy to deduce that in this example the optimal User strategy is 
\begin{equation} h  = \begin{cases}
    (+1,-1) & \text{if } \ p_{\pp } > p_{\pp \rr} \\ 
    (-1,-1) & \text{otherwise} 
\end{cases}
\label{eq:optimalUserStrategy}\end{equation}



==> modular.tex <==

\section{Modular Functions: Full-Information and the Learning Settings}
\nir{would this be better placed as the first section in the appendix? before proofs} 
\ganesh{I dont think we need this section. This is a old proof I wrote long back. }
Let $X = \{x_1, \ldots, x_L\}$ be collection a collection of sets; each set corresponding to an item. Also, let $x_{i} = \{x_{i,1}, \ldots, x_{i,p}\}$, that is an element in $x_i$ is denoted as $x_{i,j}$, and associate weight $w_{i,j}$ with each element $x_{i,j}$. Throughout this section we consider that the User's value  function is modular; that is  there exists weights $\{w\}_{i,j} \in \mathbb{R}^{pL}$ such that 
$v(x) = sign(\sum_{j } w_{ij} \mathbbm{1}(x_{i,j} \in x) )$ for all $x \in X$.

%Finally, let $\overline{X} = \{x_{i,j}\}_{i\in [L],j\in [p]}$. Since $\overline{X}$ is a set, we remove repetitions, and hence $|\overline{X}| \leq pL$. Note that elements in $X$ can be represented as unique binary vectors in $\{0,1\}^{|\overline{X}|}$. We overload notation $x_i$ to also refer to the corresponding binary vector in $\{0,1\}^{\overline{X}}$. The elements of the representation space are subsets of elements in $X$, that is for every $z \in Z$, there is an $x \in X$ such that $z\subset x$. Hence, elements in $Z$ can be represented as unique binary vectors in $\{0,1\}^{|\overline{X}|}$. %\nir{note that $v$ can be expressed as a modular threshold function: $w_p=1, w_r=-2$}

\subsection{Full-Information Setting}
Given access to $D$ and $v$, we wish to determine 
$$ h^{\star} = \argmax_{h\in \mathcal{H}}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h(\phi_h(x)) = v(x)\}]\}.$$
%From Lemma \toref this equivalent to determining 
%$$ h^* = \argmax_{h'\in \mathcal{H'}}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h'(x) = v(x)\}]\}~.$$
%From henceforth, we assume without loss of generality $h^* \in \mathcal{H}'$. We use Lemma \toref to claim that the problem reduces to the following optimization problem.\\

%\textbf{Optimization Problem}: A size 2 signed partition of $\overline{\mathcal{X}}$ is the size $2$ partition of $\overline{\mathcal{X}}$ with all elements in a partition either labelled $+$ or $-$.  Let $\mathcal{P}$ denote the set of all size 2 signed-partitions of $\overline{\mathcal{X}}$, and let $u\in \mathbb{R}_{\geq 0}$ and $v \in \mathbb{R}_{<0}$ such that $u > |(k-1)v|$. Corresponding to every signed-partition $p = \{P_+, P_-\}$, where all elements in $P_+$ are labelled $+$ and all elements in $P_-$ are labelled $-$, define a weight vector $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$ and $h'$ such that the entries of $w$ are either $u$ or $v$ and $h'(x) = \text{sign} \langle w,x\rangle$. Note that corresponding to every signed-partition there is a unique $w$ and $h'$. The objective is to determine the signed-partition corresponding to $h^*$.  

\iffalse 
\textbf{Algorithm}: We now present an algorithm that solves the above problem. For a vector in $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$ and $z \in \overline{\mathcal{X}}$, we use $w(z)$ to indicate the element of $w$ corresponding to $z$.
\begin{enumerate}
    \item Initialize $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$ to all zeros. The algorithm outputs $w$ at the end. Fix $u\in \mathbb{R}_{\geq 0}$ and $v \in \mathbb{R}_{<0}$ such that $u > |(k-1)v|$.
    \item Also initialize and $\text{Prob-wt}$ as a two-dimensional list. Each $z\in \overline{\mathcal{X}}$ has a unique row/list corresponding to it in $\text{Prob-wt}$. We use $\text{Prob-wt}(z)$ to denote the list corresponding to $z$ 
    \item Let $\mathcal{X}^+ = \{x\in \mathcal{X} \mid v(x)=1\}$ and $\mathcal{X}^- = \{x\in \mathcal{X} \mid v(x)=-1\}$
    \item For all $x\in \mathcal{X}^-$ do the following -- For all $z\in \overline{\mathcal{X}}$ such that $\{z\} \subset x$: a) Prob-wt($z$).append($x$), b) $w(z) = a_{-}$
    \item For all $x\in \mathcal{X}^+$ do the following --
    \begin{enumerate}
        \item If there exists $z\in \overline{\mathcal{X}}$ such that $\{z\} \subset x$ and $w(z) = 0$ then make $w(z) = a^{+}$.
        \item Else for all $z\in \overline{\mathcal{X}}$ such that $\{z\} \subset x$: Prob-wt($z$).append($x$).
    \end{enumerate}
    \item For all $z\in \overline{\mathcal{X}}$ determine $q(z) = \sum_{x \in \text{Prob-wt}(z)} D(x)w(z)$. Here $D(x)$ is the weight of probability on $x$.
    \item Repeat Until for all $z\in \overline{\mathcal{X}}$, $q(z) <0$:
    \begin{enumerate}
        \item Choose $z^* = \argmax_{z\in \overline{\mathcal{X}}} q(z)$ 
        \item Make $w(z^*) = v$ \ganesh{$v$ is $a^{+}$ right?  }
        \item For all $z\in \overline{\mathcal{X}}$ remove $\text{Prob-wt}(z^*)$ from $\text{Prob-wt}(z)$. 
        \item Recompute $q(z)$ for all $z\in \overline{\mathcal{X}}$ as done previously with the new $\text{Prob-wt}(z)$.
    \end{enumerate}
    \item Return $w$
\end{enumerate}
\fi 

\begin{center}
\begin{algorithm}[H]
    %\SetAlgoNoLine
    \renewcommand{\thealgocf}{}
    \DontPrintSemicolon
%    \SetAlgorithmName{$\textsc{Alg}$}{ }{ }
    \caption{$\textsc{Alg}$}
% \textbf{Output:} User optimal choice function $h$
% \;

  Let $ X^{+} := \{x| v(x) = +1\} ,  X^{-} := \{x|v(x) = -1\}$   and  $\mathcal{Z}^{'} = \{z \in \mathcal{Z}: |z| =1\}$\\ 
   \textbf{Initialize:}  $\boldsymbol{u} = \boldsymbol{0} \in \mathbb{R}^{n}$,  $\mathcal{X}_z = \phi$ for all $z\in \mathcal{Z'}$, and $\mathcal{S} = \phi$ \\
 \For{$x \in X^{-} $}{
$\boldsymbol{u}(z) = a^{-}$ for all $z\subseteq x$ and $z \in \mathcal{Z}^{'}$\\
For all $z\in \mathcal{Z'}$, and $z \subseteq x$ add $x$ to $\mathcal{X}_z$.
 }
  \For{$x \in X^{+} $}{
  \If{ exists $z \in \mathcal{Z}^{'}$ such that $z\subset x$ and $\boldsymbol{u}(z) \geq 0$}{
  $\boldsymbol{u}(z) = a^{+}$ for all $z \subseteq x$ such that  $\boldsymbol{u}(z) = 0 $ and $ z \in \mathcal{Z}^{'}$
  }
  \Else{
  For all $z\in \mathcal{Z'}$, and $z \subseteq x$ add $x$ to $\mathcal{X}_z$, and $z$ to $\mathcal{S}$ (if not already added to $\mathcal{S}$)
  }
 }
%\textcolor{gray}{Note: a) $\mathcal{S}$ is a subset of $\mathcal{Z}'$, and b) for all $z \in \mathcal{Z}'\setminus \mathcal{S}$ if $\boldsymbol{u}(z) = a^+$ then for all $x\in \mathcal{X}$ such that $z\subset x$ we have $v(x) = 1$.}\;
Let $q(z)=\sum_{x \in \mathcal{X}_z}D(x)v(x)$ for all $z \in \mathcal{S}$\;
\inbal{$q$ overload?}
% \ןמנשף

\While{there does not exist $z  \in   \mathcal{S}$ such that $q(z) \geq 0$}{
Let $z^{\star} = \arg \max_{z \in \mathcal{S}} q(z) $\\
$\boldsymbol{u}(z^*) = a^+$\\
$\mathcal{S} = \mathcal{S}\setminus {z^{\star}}$\\
 $\mathcal{X}_z = \mathcal{X}_z \setminus \mathcal{X}_{z^{\star}}$ for all $z \in \mathcal{S}$\\
Recompute $q(z)$ for all $z\in \mathcal{S}$
}
\Return $\boldsymbol u $
\end{algorithm}
\end{center}
\iffalse 
Now we try to argue the correctness. First let us define the following sets:

a) $\mathcal{X}^{++} = \{x\in \mathcal{X}^+ \mid \text{ there exists } z\in \mathcal{Z}' \text{ such that } z\subset x \text{ and for all } x' \in \mathcal{X}^{-}, \ z \nsubseteq x'\}$

b) $\mathcal{X}^{--} = \{x\in \mathcal{X}^- \mid \text{ for all } z\in \mathcal{Z}' \text{ such that } z\subset x,\ z \notin \mathcal{S}\}$

\begin{lemma}
For every $x \in \mathcal{X}^{++} \cup \mathcal{X}^{--}$ we have $h(\phi_h(x))  = v(x)$.
\end{lemma}
\begin{proof}
Case a) $x \in \mathcal{X}^{++}$: For all such $x$ step 11 is executed which ensures $h(x) =1 = v(x)$. It is easy to verify that thereafter in the algorithm $h(x)$ remains equal to $1$ for all $x\in \mathcal{X}^{++}$. \\

Case b) $x \in \mathcal{X}^{--}$: Since $\mathcal{X}^{--} \subseteq \mathcal{X}^{-}$, we have at the end of step 6, $h(x) = -1 = v(x)$ for all $x \in \mathcal{X}^{--}$. Additionally since for all $z\in \mathcal{Z}$ such that  $z\subset x$, $z \notin \mathcal{S}$ in the remaining steps $h(x)$ continues to be equal to $-1$. 
\end{proof}

We will employ the potential function argument to show that the algorithm computes $h$ which is optimal. To this end let us define for any subset $\mathcal{U} \subseteq \mathcal{X}$ and a $h' \in \mathcal{H}'$ 
$$\text{Pot}(\mathcal{U}, h') = \sum_{x \in \mathcal{U}} D(x) \cdot \mathbbm{1}\{h'(\phi_{h'}(x) = v(x)\} $$
Note that $\text{Pot}(\mathcal{X}, h')$ is the utility of $h'$. From the above lemma we have that for any $h'\in \mathcal{H}'$ and $h$ output by our algorithm the following is satisfied:
$$\text{Pot}(\mathcal{X}^{++} \cup \mathcal{X}^{--}, h) \geq \text{Pot}(\mathcal{X}^{++} \cup \mathcal{X}^{--}, h')  $$

Let $z_t^*$ be the solution of the arg max at end of the $t$-th iteration of the loop (steps 19-24). Note that  $\mathcal{X}_{z_1^*}$, $\mathcal{X}_{z_2^*}, \ldots , \mathcal{X}_{z_t^*}$ are disjoint sets (owing to step 3). Let 
$$\mathcal{U} = \mathcal{X}^{++} \cup \mathcal{X}^{--} \cup \mathcal{X}_{z_1^*} \cup \mathcal{X}_{z_2^*} \cup \ldots \cup \mathcal{X}_{z_t^*}$$ at the end of $t$-th iteration. Then we will show for every $t$ and $h' \in \mathcal{H}'$
$$\text{Pot}(\mathcal{U}_t, h) \geq \text{Pot}(\mathcal{U}_t, h')$$
\fi 
We construct the User's choice function from $\boldsymbol u$ as follows,  $$h(z) = \text{sign} \Big(\sum_{z' \in \mathcal{Z}^{'} \cap z} \boldsymbol{u}(z') \Big) \ \ \ \text{ for all} z \subseteq  \mathcal{Z}.$$

\subsection{Proof of optimality and correctness}
We begin with the following lemmas. 
\begin{restatable}{lemma}{userPayoff}
   $ \mathcal{U}(h) :=   \frac{1}{2} \cdot \sum_{x \sim D(X)} \sum_{z|\phi_{h}(x) = z}h(z)\cdot v(x)   + \frac{1}{2} $
   \label{lem:userPayoff}
\end{restatable}
Using Lemma 1, throughout this proof, we assume without loss of generality,  that the representations $\phi_{h}(x)$ for each $x$ are assigned according to the order in which choice function value $a^{+}$ is assigned by the algorithm. First, note that the set  $\mathcal{S}$ at the end of line \toref{ } can be characterized by,      \begin{align}
\mathcal{S} = \{z^{'} \in \mathcal{Z}^{'} &| \exists x \in X_{z^{'}} \text{ such that } v(x) = +1 \nonumber \\ &\text{ and } \boldsymbol{u}(z) = a^{-} \text{ for all } z \in Z_x \}
\end{align}

 Next, we observe that, since $a^{+} \geq |n-1|a^{-}$,  for any atomic  representation $z^{'}$ with  weight $a^{+}$, all representations that consist it will have $h(z) = +1$. Formally,


\begin{lemma}
For every $z \in \mathcal{Z}$ we have $h(z)  = +1$ iff there exists $ z^{'} \in \mathcal{Z}^{'}$ and $z^{'} \subseteq z$ such that $\boldsymbol u (z') = a^{+}  $ and $h(z)  = -1$ otherwise.
\label{lem:Positive}
\end{lemma}
\begin{proof}[Proof of Optimality]
Observe that the User's payoff function given in Lemma \ref{lem:userPayoff}  can be rewritten as \\ 
$$ \frac{1}{2} \sum_{z \in \mathcal{Z}} \sum_{x \in  \phi_{h}^{-1}(z)} D(x) v(x) h(z) + \frac{1}{2}
$$
\textbf{Case 1 ($z \notin \mathcal{S}$ and $\phi_{h}^{-1}(z) \neq \emptyset$):}  For every $x \in \phi_{h}^{-1}(z) \cap X^{-} $ we have   $\boldsymbol{u}(z')= a^{-}$ for all $z' \in \mathcal{Z}^{'} \cap x $ (Line 6).
This gives 
$$h(z) = \text{sign}\Big(\sum_{z^{'} \in \mathcal{Z}^{'} \cap z } \boldsymbol{u}(z^{'}) \Big) = \text{sign} \Big(  \sum_{z^{'} \in \mathcal{Z}^{'} \cap z } a^{-} \Big) = -1  $$

The User gets a payoff of $\sum_{x \in \phi_{h}^{-1}(z) }D(x) v(x)h(z) = \sum_{x \in \phi_{h}^{-1}(z) }D(x) (-1)(-1) = \sum_{x \in \phi_{h}^{-1}(z) }D(x).$     Otherwise, if $x \in \phi_{h}^{-1}(z) \cap X^{+}$ we have that there is  $z' \subset x$ such that $ \boldsymbol{u}(z') = a^{+}$ (Line 10). Let $M = \{z^{'} \in x \cap z \cap \mathcal{Z}^{'}| \boldsymbol{u}(z^{'}) = a^{+} \}$ and note that $M \geq 1$, we have  
\begin{align*}
    h(z) &= \text{sign}\Big( \sum_{z' \in \mathcal{Z}^{'} \cap z } \boldsymbol{u}(z^{'})\Big) \\ 
    & = \text{sign}\Big( \sum_{z^{'} \in M } a^{+} +  \sum_{z^{'} \in \mathcal{Z}^{'} \cap z \setminus M } a^{-} \Big)  \\ 
    & = +1   \tag{Lemma \ref{lem:Positive}}
\end{align*}
 In this case,  User's payoff  is given as  $ \sum_{x \in \phi_{h}^{-1}(z)}D(x)h(z)v(x) = \sum_{x \in \phi_{h}^{-1}(z)}D(x)(+1)(+1) = \sum_{x \in \phi_{h}^{-1}(z)}D(x)$. Otherwise, if $|M| = 0$ then $h(z) = -1$ and $h(z') = +1$ for some $z^{'} \not \subset z$ and hence  $z$ is not a best response of System i.e. $z \neq \phi_h(x)$, contradicting the assumption  that $x \in \phi_{h}^{-1}(z)$. 

\textbf{Case 2 ($ z \in \mathcal{S}$ and $ \phi_{h}^{-1}(z) \neq \emptyset$):} We have following two sub-cases: either $q(z) < 0$ or $q(z)\geq 0$ at the end of execution of the algorithm. In the first case, the algorithm does not update  the choice function after initial assignment  in Lines 6   and hence $q(z) < 0$ for every step in the while loop(Line 18). Furthermore,  we have   $h(z) = -1$ and $v(x) = -1$ for all $x \in \phi_{h}^{-1}(z)$ (see Line 6).  Hence, User's payoff is given as $\sum_{x \in \phi_{h}^{-1}(z)}D(x)$.   

We now show that if $q(z) \geq 0$, the algorithm finds an optimal representation. Let $z_{1}^{\star}, z_2^{\star}, \cdots , z_{m}^{\star}$ be the sequence in which the algorithm assigns the weight $a^{+}$ in Line 20 and let $z_{\ell}^{\star}$ be the first singleton representation that is in $z$. Then, as $\boldsymbol{u}(z_{\ell}^{\star}) = a^{+}$, we have from Lemma 3 that $h(z) = +1$. Furthermore, we have for all $x \in \mathcal{X}_{z}$ such that $\phi_{h}(x) \neq z$ that,  there is a $z^{\star} \not\subset z$ such that $\boldsymbol{u}(z^{\star}) = a^{+}$. Hence, following the sequence of best response assignments we have  $z^{\star} \in \{z_{1}^{\star}, \cdots, z_{\ell -1}^{\star} \}$ and  $\mathcal{X}_{z^{\star}} = \phi_{h}^{-1}(z^{\star}) $. This implies  $ q_{z^{\star}} \geq q_{z_{\ell}^{\star}}$ and    $$\sum_{x \in \phi_{h}^{-1}(z^{\star})} D(x) \geq \sum_{x \in \phi_{h}^{-1}(z_{\ell}^{\star})} D(x).  $$
The above expression gives that for every representation $z$ we have that it gives a maximum payoff of $ \sum_{x \in \phi_{h}^{-1}(z_{\ell}^{\star})} D(x)$ to the User. This completes the proof of the theorem.  
%First note that in Line 18 we have $h(z) = -1$ and, 
%\begin{align*}
 %   q(z)h(z) &=  (\sum_{x \in \mathcal{X}_{z} \cap X^{+}} D(x) -  \sum_{x \in \mathcal{X}_{z} \cap X^{-}} D(x)) h(z) 
  %  =  \sum_{x \in \mathcal{X}_{z} \cap X^{-}} D(x) -  \sum_{x \in \mathcal{X}_{z} \cap X^{+}} D(x) \leq 0
%\end{align*}
%Next observe that 
%This implies $\sum_{x \in \mathcal{X}_{z} \cap X^{-}}D(x) > \sum_{x \in \mathcal{X}_{z} \cap X^{+}}D(x) $

%we have $z^{\star} \in \mathcal{S} \subseteq \mathcal{Z}^{'}$ such that $\boldsymbol{u}(z^{\star}) = a^{+} $. Using the same argument used for the first case we have $h(z) = +1$ and User payoff is given as 
%$\sum_{x \in \phi_{h}^{-1}(z)}D(x)$. On the other hand if $q(z) < 0 $ we have that 
\end{proof}

\iffalse 
\begin{lemma}
  $q(z)\boldsymbol{u}(z) < 0 $ iff $q(z) > 0$ and $\boldsymbol u (z) <0$.
\end{lemma}
\begin{proof}
Say, for contradiction, that $ \boldsymbol u(z) > 0$ and $q(z) < 0$. This implies that for at-least one $x \in X_z$ we have $v(x) = -1$. This means that $\boldsymbol{u}(z) = a^{-} < 0$ which is a contradiction. 
\end{proof}
\begin{lemma}
Let $z \in \phi_{h}(x)$ for some $x$ and $z \notin \mathcal{Z}^{'}$.  Then there is $z^{'} \in \mathcal{Z}^{'}$ such that $z' \subseteq z$ and $ z^{'} \in  \phi_{h}(x)$.
\end{lemma}
\begin{proof}
Let $h(z) = -1$ then by Lemma \toref we have that for all  $z^{'} \subseteq z$ we have $ h(z^{'}) = -1$. Hence every $z^{'}$ is also a best response. On the other hand  if $h(z) = +1$ then by Lemma \toref we have that there is a $z^{'} \subseteq z$ such that $h(z^{'}) = +1 $ hence $z^{'} \in \phi_{h}(x)$.  
\end{proof}
The above lemma shows that without loss of generality we can restrict our attention to $\mathcal{Z}^{'}$. Hence we can rewrite the User's payoff as 
$$\mathcal{U}(h) = \sum_{z^{'} \in \mathcal{Z}^{'}} \sum_{x| \phi_{h}(x) = z^{'}} D(x) v(x) h(z^{'}) $$
\ganesh{ Proof incomplete! }
\fi 

\subsection{ The Learning Problem}

Let $v: \mathcal{X} \rightarrow \{-1,1\}$ be the value function. We restrict our attention to the hypothesis class $\mathcal{H}$ consisting of modular functions. In particular for each $h\in \mathcal{H}$ there is a $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$, such that $h(z) = \text{sign}(w^Tz)$. Further, Let $\mathcal{H}' = \{h' \mid \text{ there exists } h \text{ such that } h(\phi_h(x_i)) = h'(x_i) \text{ for all } x_i\}$. \\

\begin{restatable}{lemma}{SVC}
For every $h^{'} \in \mathcal{H}^{'}$ we have $h^{'}(\phi_{h^{'}}(x)) = h^{'}(x)$.
\end{restatable}



\begin{restatable}{lemma}{modular}
Let $\mathcal{J} = \{h \in \mathcal{H}: h(x') =-1 \text{ for all } x^{'} \subseteq x \text{ if } h(x) =-1 \}$ and let the representation space consists of subsets of size at most k then, $ \mathcal{H}^{'} = \mathcal{J}$. In particular $\mathcal{H}'$ is a strict subset of $\mathcal{H}$ (if $\mathcal{H}$ is modular).
\end{restatable} 

From here on we assume the representation space consists of subsets of size at most $k$.
\begin{lemma}
Let $\mathcal{H}$ and $\mathcal{H}'$ be as above. Then the following holds:
$$ \max_{h \in \mathcal{H}}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h(\phi_h(x)) = v(x)\}]\} = \max_{h' \in \mathcal{H}'}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h'(x) = v(x)\}]\}~.$$
\end{lemma}
\begin{proof}
From Lemma \toref\ and since $\mathcal{H}'$ is a strict subset of $\mathcal{H}$, it follows that 
$$ \max_{h \in \mathcal{H}}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h(\phi_h(x)) = v(x)\}]\} \geq \max_{h' \in \mathcal{H}'}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h'(x) = v(x)\}]\}~.$$
Let $h^{\star} = \argmax_{h \in \mathcal{H}}\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h(\phi_h(x)) = v(x)\}]\}$. From the construction of $\mathcal{H}'$, there is a $h' \in \mathcal{H}'$ such that $h(\phi_h(x)) = h'(x)$ and 
$$\{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h^{\star}(\phi_{h^{\star}}(x)) = v(x)\}]\} = \{\mathbb{E}_{x \sim D}[\mathbbm{1}\{h'(x) = v(x)\}]\}~.$$
Since $h'\in \mathcal{H}'$, the lemma follows.
\end{proof}

\begin{lemma}
Let $a_{+}\in \mathbb{R}_{\geq 0}$ and $a_{-} \in \mathbb{R}_{<0}$ such that $a_{+} > |(k-1)a_{-}|$. Then corresponding to every $h'\in \mathcal{H}'$ there is a $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$ such that the entries of $w$ are either $a_{+}$ or $a_{-}$ and $h'(x) = \text{sign} \langle w,x\rangle$.
\end{lemma}
\begin{proof}
Let $h' \in \mathcal{H}'$. For every $x$ such that $h'(x) = -1$ let the values of $w$ corresponding to elements in $x$ be $a_{-}$. Let all the remaining values of $w$ be equal to $a_{+}$. It follows from Lemma \toref that $h'(x) = \text{sign}(\langle w,x\rangle)$ for all $x\in \mathcal{X}$.
\end{proof}

\iffalse
Let $\mathcal{X} = \{x_1, \ldots, x_L\}$ be collection a collection of sets; each set corresponding to an item. Also, let $x_{i} = \{x_{i,1}, \ldots, x_{i,p}\}$, that is an element in $x_i$ is denoted as $x_{i,j}$, and associate weight $w_{i,j}$ with each element $x_{i,j}$. Finally, let $\overline{\mathcal{X}} = \{x_{i,j}\}_{i\in [L],j\in [p]}$. Since $\overline{\mathcal{X}}$ is a set, we remove repetitions, and hence $|\overline{\mathcal{X}}| \leq pL$. Note that elements in $\mathcal{X}$ can be represented as unique binary vectors in $\{0,1\}^{|\overline{\mathcal{X}}|}$. We overload notation $x_i$ to also refer to the corresponding binary vector in $\{0,1\}^{\overline{\mathcal{X}}}$. The elements of the representation space are subsets of elements in $\mathcal{X}$, that is for every $z \in \mathcal{Z}$, there is an $x \in \mathcal{X}$ such that $z\subset x$. Hence, elements in $\mathcal{Z}$ can be represented as unique binary vectors in $\{0,1\}^{|\overline{\mathcal{X}}|}$.

For every $x\in \mathcal{X}$ and $z\in \mathcal{Z}$, define $v(x) = \text{sign}(w^Tx_i)$ and $v(z) = \text{sign}(w^Tz)$ respectively, where $w = (w_{i,j}) \in \mathbb{R}^{|\overline{\mathcal{X}}|}$. 

\textbf{Learning Problem}: The user has access to the training set $T =\{(x_1,v(x_1), \ldots, (x_n, v(x_n))\}$, where the points $x_1, \ldots , x_n$ are sampled iid according to the unknown distribution $D$. \\

\textbf{Hypothesis class}: We restrict our attention to the hypothesis class $\mathcal{H}$ consisting of modular functions. In particular for each $h\in \mathcal{H}$ there is a $w \in \mathbb{R}^{|\overline{\mathcal{X}}|}$, such that $h(z) = \text{sign}(w^Tz)$. \\ 

\textbf{Naive ERM Learning}: Learn $w$'s to minimize the empirical loss, that is, $\arg \min_{w} \sum_{i\in [n]}\text{sign}(w^Tx_i) \neq v(x_i)$. Assuming the existence of truthful representations and benevolent systems, we have statistical guarantees for naive learner. The statistical guarantee depends on $|\overline{\mathcal{X}}|$, which is the VC dimension of the $\mathcal{H}$.\\

\textbf{Strategic ERM Learning}: We know every $u \in \mathbb{R}^{|\overline{\mathcal{X}}|}$ defines a $h$. Learn $u$'s to minimize the \emph{strategic}-empirical loss, that is, $\arg \min_{u} \sum_{i\in [n]} h(\phi_h(x_i)) \neq v(x_i)$. \\

Let $\mathcal{H}' = \{h' \mid \text{ there exists } h \text{ such that } h(\phi_h(x_i)) = h'(x_i) \text{ for all } x_i\}$. We wish to essentially learn $\mathcal{H}'$. 

Let $\mathcal{H}$ be the class of modular functions, where every $h \in \mathcal{H}$ satisfies truthful representation assumption.
It is important to note that $h'$ is a set-function.

\ganesh{One immediate consequence of above construction is the following lemma. 

\begin{lemma}
For every $h^{'} \in \mathcal{H}^{'}$ we have $h^{'}(\phi_{h^{'}}(x)) = h^{'}(x)$.
\end{lemma}
\begin{proof}
By construction we have 
$$ h^{'}(\phi_{h^{'}}(x)) = h(\phi_{h}(\phi_{h^{'}}(x))) \text{ for some } h \in \mathcal{H}$$
Note that since $h$ is modular, any representation of $\phi_{h^{'}}(x)$ is also a representation of $x$. Also as $\phi_{h^{'}}(x)$ is a strategic representation of itself. Hence, we have 
\begin{align*} h^{'}(\phi_{h^{'}}(x)) = h(\phi_{h}(\phi_{h^{'}}(x))) &= \text{sign}(\langle \boldsymbol{u}, \phi_{h}(\phi_{h^{'}}(x)) \rangle ) \\ &= \text{sign}(\langle \boldsymbol{u}, \phi_{h}(x)\rangle ) \\ &= h(\phi_h(x)) \\&= h^{'}(x)\end{align*}
\end{proof}
}

Questions: a) What is $\mathcal{H}'$ if $\mathcal{H}$ is modular?\\
b) What is computational complexity of the strategic ERM in the case of modular functions?

\begin{lemma}
Let the representation space $\mathcal{Z}$ consist of subsets of size at most $k$. Then $\mathcal{H}'$ is modular. 
\end{lemma}
\begin{proof}
It is sufficient to show that $h'$ corresponding to every $h\in \mathcal{H}$ is modular. Let $h$ and $u$ be such that $h(x) = \text{sign}(\mathbf{u}^Tx)$. First observe that if $h(x) =1$ then $h'(x) =1$: as there exists a $z \subseteq x$ such that $\text{sign}(\mathbf{u}^Tz) = 1$ (take the singleton indexed by the maximum element in $u$ restricted to $x$). Further, if $h(x) = -1$ and $h'(x) = -1$ then all the elements of $u$ restricted to restricted to $x$ are $\leq 0$; in particular for all $z\subseteq x$ we have $\text{sign}(\mathbf{u}^Tz) = -1$. Hence, we only care about the case when $h(x) = -1$ and $h'(x) = 1$. This implies there exists a singleton $z \subset x$ such that $\text{sign}(\mathbf{u}^Tz) = 1$. We note that for all $x'$ such that $z \subset x$ we have $h(x') =1$. Since the $z$ is a singleton, we can increase the element in $u$ corresponding to $z$ and obtain $u'$ such that $\text{sign}((u')^Tx) = 1$.
\end{proof}


\begin{lemma}
Let the representation space $\mathcal{Z}$ consist of subsets of size at most $k$. Then $\mathcal{H}'$ is a strict subset of $\mathcal{H}$, and $\mathcal{H}' = \{h' \mid \text{there exists } u' \text{ such that } h'(x) = \text{sign}(<u',x'>) \text{ and if }  \text{sign}(<u',x'>) = -1 \text{ then all the elements of } u' \text{ restricted to } x' \text{ is } \leq 0 \}$. 
\end{lemma}
\begin{proof}
The proof . . 
\end{proof}
\ganesh{ Define $\mathcal{J} = \{h \in \mathcal{H}: h(x') =-1 \text{ for all } x^{'} \subseteq x \text{ if } h(x) =-1 \}$.  \begin{lemma}
Let $\mathcal{H}$ be modular and representation space consists of subsets of size at most k then, $ \mathcal{H}^{'} = \mathcal{J}$.
\end{lemma} 
\begin{proof}
Let $h^{'} \in \mathcal{H}^{'}$ and, for contradiction assume that $h^{'} \notin \mathcal{J}$. Hence, there exists some $x$ and $x^{'} \subseteq x$ such that $h^{'}(x) = -1$ and $h^{'}(x^{'}) = +1$. Since $h^{'} \in \mathcal{H}^{'}$, we have $h^{'}(x^{'}) = h(\phi_{h}(x^{'})) = +1$ for some $h\in \mathcal{H}$. As the representation space consists of at most $k$ elements every representation of $x^{'}$ is a valid representation of $x$. Hence, we have $ +1 = h(\phi_{h}(x^{'})) = h(\phi_{h}(x)) = h^{'}(x) $, a contradiction. We have $\mathcal{H} \subseteq \mathcal{J}$. 

On the other hand, to show that $\mathcal{J} \subseteq \mathcal{H}^{'}$ it is enough to show that for every $h^{'} \in \mathcal{J}$  there is an  $h \in \mathcal{H}$ such that $h(\phi_{h}(x)) = h^{'}(x)$ for all $x$. In particular, for $h = h^{'}$ this condition is satisfied. 
\end{proof}  }
\fi

\subsection{PAC Learning}
The learning objective in strategic representation is   minimizing  strategic error given by    $$ \texttt{err}_S(h) := \mathbb{E}_{x \sim D}[h(\phi_h(x)) \neq v(x)  ].$$

Call the optimal representation as $h^{\star}$. Let the sample error be represented by 
$$\widehat{\texttt{err}_S}(h) := \frac{1}{n} \sum_{ i \in [n] }\mathbbm{1}[h(\phi_h(x_i)) \neq v(x_i) ].$$

%\paragraph{Learning Agnostic User strategy:} Given $n$ i.i.d. data point  $S_n = \{x_i, v(x_i)\}_{i=1}^{n}$ sampled from a  distribution $D$ and labelled by the value function (\ganesh{We can even consider a joint distribution over $D \times \{-1,1\}$}), the problem is to learn the policy $h_{agn}$. Since $h_{agn}$ depends only on $\mathbb{P}(X^{+})$, one can efficiently learn it using standard PAC bounds. For instance, using  Hoeffding's inequality to bound the error probability (See Appendix \toref{}) 

%\section{Lower bound}
%Consider that the System has access to the  oracle that takes $z \in \mathcal{Z}$ as  input and returns $h(z)$. Furthermore, as stated  earlier, consider that the value function is modular $v(x) = \sign(\sum_{i\in[n]} w_{(i)})$.    We show that System requires $\Omega  ({n \choose k})$ queries to the oracle to compute $\phi_h(x) \in \mathcal{Z}$. First, notice that, given $x$,  the System's goal is to find $\phi_{h}(x) \in h^{-1}(1)$. Let, without loss of generality, $h^{-1}(1) \neq \emptyset $, for otherwise, any $z \subset x$ with $|z| = k $ is a best response. From the truthfulness assumption we have that $\phi_{h}(x) =   \{ x_{(1)}, x_{(2)}, \cdots x_{(k)}\}$ for some item descriptions $x_{(1)}, \cdots x_{(k)}$. %Since $h$ is chosen by the User such that $\phi_{h}(x) \in h^{-1}(v(x))$ 
%Furthermore let $v(x)=1$. %and the set $L := $\{(x_{(1)}, x_{(2)}, \cdots x_{(k)}): \sum_{i=1}^{k} w_{i} x_{(i)} > 0 \}$ is non-empty.   To see  that $L \cap h^{-1}(1) \neq \emptyset$,  observe  that $v(x) = 1 = h(\phi_{h}(x)) = h(z)$ for all $z \in L$. 
%Consider the following weights $w_i = 1$ for exactly $k$ item descriptors,  and for others weight is given as $-(k-1) $.  

\iffalse
\begin{definition}[Agnostic PAC learnability for strategic representation]
 We call a choice function class $ \mathcal{H}$  strategically learnable  by an ERM rule if, for any $\varepsilon, \delta \in  (0,1)$, we have $n_{0}(\varepsilon, \delta) \in \mathbb{N}$ such that for any $n > n_0(\varepsilon, \delta)$, for any distribution $D$ over $X$, for any value function $v:X \rightarrow \{0,1\}$ and for any representation relation $R: X \rightarrow 2^Z$ we have that $\mathbbm{P}_{x \sim X}\{  \widehat{\texttt{err}}_S (h) -\texttt{err}_S (h^{\star})   >  \varepsilon   \}  \leq \delta $. Here, $h$ is a choice function returned by the ERM rule over $n$ i.i.d. samples from $D$. 
\end{definition}
\paragraph{Example 1 continued:}   The learning problem in this example is to determine if $p_{\pp } > p_{\pp\rr}$. Without loss of generality consider that $p_{\pp } > p_{\pp\rr}$ (the proof when $p_{\pp } < p_{\pp\rr}$ is similar). 

Given a training set $T = \{x_{i}\}_{i=1}^{n}$,  let $\widehat{p}_{x} = \frac{1}{n} \sum_{i=1}^{n} \mathbbm{1}(x_i =x)$ denote an empirical mean for $ x \in X$.  Consider the User strategy with $\widehat{D} := (\widehat{p}_{x})_{x \in X}$ in \textsc{Alg}.  

In our example we have  
\begin{equation*}
    h := \begin{cases}
    (+1, -1)  & \text{if}  \ \widehat{p}_{\pp} - \widehat{p}_{\pp\rr} >  \varepsilon_{n} \\
    (-1, -1) & \text{otherwise}
    \end{cases}
\end{equation*}
\fi 

\section{TODO} 

\textbf{outline:} 
\\ main storyline: naïve vs strategic users
\\ users: knowledge - v; power - choose H, commit to h
\\ system: power - subset sizes k1-k2
show that being naïve can be really bad
\\ show that being strategic can help - by showing that it's possible to learn: 
computationally
statistically
in absolute terms
\\ main point: balance of power (system: k1-k2;  users: H) determines expressivity and hardness
define and quantify gap between naïve and strategic
give example of really bad gap
give handle on what controls this gap (as a function of what?)
show that even mild strategizing can help (in terms of closing the gap):
let users control how much "effort" they invest in learning (by "choosing" which balance-of-power to learn in)
\\ show that more effort => smaller gap, and that this has diminishing returns
"min pain - max gain": with minimal effort, can recover most of the gap
characterize user susceptibility to manipulation
as relation/"distance" between v and H'?
fairness: when susceptibility correlates with some other attribute
consider users working together:
e.g., minimally strategic + data sharing = good for all

\text{Open Question} Intuition: Fix  User's $h$ and $v$  to be a threshold  on   sub-additive functions and look at $k=k_1=k_2$. For smaller $k$, the System has lesser reprentations to choose from. On one hand, the system can bundle many items to the same representation which may help the system to extract more surplus. On the other hand, as the User  strategically report  $h$  the cumulative  payoff of the System as it  may result increase the Systems' payoff as  larger size of representation set gives more flexibility to the System.   An open question is what happens in equilibrium.   

\subsection{List of results}
\begin{enumerate}
\item We define representation game with  strategies and sequence of play. 
    \item Lemma 1: Systems  best response strategy may  not be  unique. However, every best response strategy gives  the same payoff to the User. This allows us to write the Users payoff irrespective of specific choice of specific best response strategy used by System.  
    \item A naive user who assumes that the System acts in its best interest can be tricked by the System into choosing her  non-preferred choice. An agnostic user, on the other hand can guarantee herself the payoff of  at-least $1/2$ irrespective of the type (Benevolent,  or Strategic) of the System. 
    \item Lemma 3.1: there is a $k \in[k_1, k_2]$ such that it is enough to look only at the representations of size $k$. All $k$ sized representations are called units.  
    \item We define $k$-set modular functions  as  functions that admit   $k$-sized unit representations.
    \item A $k$-set modular function can be represented as threshold function over sum of  binary values weights over unit representations.  A  $k$-set modular function is not a $k-1$ set modular.    
    \item Let the value function is $k^{\star}$-set modular ($k^{\star}$ is the smallest value of $k$ in $k$-set modular). If $k^{\star} \leq k_2$  then strategic User can fully extract the surplus (guarantee payoff of 1).  %$k$-sized representations. 
    
    \item \textbf{Algorithmic result:} We give an algorithm (two algo but the second one is not written down) that finds an optimal $h$ for User. As a consequence of above results, if the value function is relatively simple ($k^{\star} \leq k_2$)  User can guarantee payoff of 1. We need fine grained analysis of User payoff as we increase $k^{\star} > k_2$. Algorithm runs in polynomial time (in terms of size of representation space).
    \item Learning: Define $\mathcal{H}^{'}$ as a set of representations $h^{'}$ such that strategic representation under some $h$ is non strategic one under $h^{'}$. We essentially need to learn $h^{'}$ instead of $h$. When $\mathcal{H}$ is  is modular $\mathcal{H^{'}}$ is also modular. Hence, under modular functions the problem is to find a learning  of binary valued  weight (See Point 6 above) for each representation. 
\end{enumerate}

\subsection{Missing links}
\begin{itemize}
    \item Gaps: how to go from simple $h$ to complex $h$  
    \item 
\end{itemize}

\iffalse 
\section{More Observations  (\Naive\ User) }
We considered that a \naive\  User assumes that the system is benevolent and hence does not account for any strategic manipulation from Systems'  behalf. This means that a \naive\ User reports her value function truthfully.     Here, we define a \emph{skeptical-\naive} User who resolves ties between  \naive\ truthful representations by taking into account System's best response. While the User is still \naive\ in her assumption about Systems's intentions, she wants to find a truthful strategy that is most robust to any deviation from benevolence. 
\begin{definition}[Skeptical-\naive\  User]
 The skeptical-\naive\ users choice function is given as, 
 $$h_{\texttt{S-\Naive}} \in \argmax \limits_{  h \in \{\text{truthful}\} } \mathbb{E}_{x \sim D} \mathbbm{1}[h(\phi_{h}(z)) = v(x)] $$
\end{definition}

\paragraph{Example 1 continued:} Recall that in the example we designed a worst case distribution for a given truthful strategy. A choice function of a skeptical-\naive\ User, however, depends on the distribution as follows, 
\begin{align*}
    h_{\textsc{S-Naive}} = \begin{cases}
    (+1,+1,-1) &\text{If }  \mathbb{P}(\mathcal{X}^{+} \geq \mathcal{X}^{-}) \\
    (+1,-1,-1) & \text{If } \mathbb{P}(\X^{-} > \X^{+}) \text{and } \Prob(x_2) \geq \Prob(x_3) \\ 
    (-1,+1,-1) & \text{If} \mathbb{P}(\X^{-} > \X^{+}) \text{and } \Prob(x_3) > \Prob(x_2)
     \end{cases}
\end{align*}
A skeptical-\naive\ Users  payoff when facing a strategic System is given as, 
\begin{align*}
    \mathcal{U}(h_{\texttt{S-Naive}}) &= \Prob(x_1) + \mathbbm{1}[\Prob(\X^{-}) >  \Prob(\X^{+})]\big( (\Prob(x_2) \cdot   \mathbbm{1}[\Prob(x_2) \geq \Prob(x_3)] + \Prob(x_3) \cdot   \mathbbm{1}[\Prob(x_3) > \Prob(x_2)] \big) \\
    & =  \Prob(x_1) + \mathbbm{1}[\Prob(\X^{-}) >  \Prob(\X^{+})]\max(\Prob(x_3),  \Prob(x_2))\geq 1/2
\end{align*}

The idea is to \emph{guard} against worst case instance of manipulation by the strategic System. This can be extended to the general setting to get the following result. 
\begin{lemma}
Given a strategic representation instance, a skeptical-\naive\ user guarantees for herself the payoff of at-least 1/2.  
\end{lemma}
\fi

==> moved_stuff.tex <==
\section{\red{MOVED STUFF}}

\subsection{\red{Stuff moved from Sec. 4.2}}
\paragraph{Lifted functions.}
The relation between choice functions and their induced counterparts
passes through an additional type of functions that operate
on sets of size \emph{exactly} $\ell$.
Denote $\Z_\ell = \{z \in \Z : |z| =\ell\}$,
and note that all feasible representations can be partitioned as
$\Z = \Z_{k_1} \uplus \ldots \uplus \Z_{k_2}$.
We refer to functions that operate on single-sized sets 
as \emph{restricted functions}.
Our next result shows that choice functions of order $k$
can be represented by restricted functions over $\Z_k$ that are `lifted' to operate on the entire $\Z$ space.
\begin{lemma}\label{lemma: h in H_k are lifts on size at most k}
For each $h \in H_k$
there exists a corresponding $g: Z_{k} \rightarrow \pmone$
such that $h = \lift(g)$, where:
\begin{equation*}
\lift(g)(z) =
    \begin{cases}
        1 & \text{\textnormal{if }} k \le |z| \text{\textnormal{ and }} \\
        & \exists z' \subseteq z, |z'|=k \,\text{\textnormal{ s.t. }}\, g(z')=1 \\
        -1 & \text{\textnormal{o.w.}}
    \end{cases}
\end{equation*}
\end{lemma}
\begin{proof}
Let $h \in H_k$.  Then there is a weight function $w$ on sets of size at most $k$ such that either $w(z) \in (-1,0)$ or $w(z)  > \sum_{i \in [k]} {n \choose i}$, and 
\[
h(z) = \sign \left( \sum\nolimits_{z':z' \subseteq z, |z'| \le k} w(z') \right)
\]
Define $g:\Z_k \rightarrow \{-1,1\}$ such that for a $z\in \Z_k$, $g(z) = 1$ if $w(z) > 0$ and $g(z) = -1$ otherwise. It is easy to see from the choice of $w(z)$ that $h = \lift(g)$.
\end{proof}
This will allow us to work only with sets of size exactly $k$.
\nir{is this true?}

% $\lift(g)(z)=$: \\
% - $k_1 < k \le k_2$: \\
% --- if $k_1 \le |z| < k$, $=-1$ \\
% --- if $k \le |z| \le k_2$, $=1$ if $\exists z' \subseteq z, |z'|=k$ s.t. $h_k(z')=1$, ow $=-1$ \\
% - $k \le k_1$: \\
% --- $=1$ if $\exists z' \subseteq z, |z'|=k$ s.t. $h_k(z')=1$, ow $=-1$
% (this is the same as the second case above)
% \todo{write cases more compactly}

\outline{• [DEF] induced $F_k$ }

---------------------------------------------------------------------
Our algorithm works directly with induced functions as these
provide direct access to loss computations,
and our next set of result show that induced functions have useful structure.
We start by relating the complexities of $h$ and $f_h$.
\begin{definition}
A function $f: \X \rightarrow \pmone$
has an \emph{induced complexity} of $\ell$
if exists a function $g:\Z_\ell \rightarrow \pmone $ s.t.:
\[
f(x) = 
\begin{cases}
        1 & \text{\textnormal{if }} \,\, \exists  z \subseteq x, |z|=\ell \,\,\text{\textnormal{and}}\,\, g(z)=1 \\
        -1 & \text{\textnormal{o.w.}}
    \end{cases}
\]
\todo{add that there exists no function $g':Z_{\ell-1} \rightarrow \pmone$ satifying the above}
\end{definition}
\todo{again this is useful to compare to $v$}

\blue{($g$ is like an $h_\ell$ that can be lifted to a corresponding $h$)}

\todo{connect complexity classes of $H$ and $F$}
\blue{Think of a function $h$ in $H_{\ell}$ but not in $H_{\ell-1}$ (we know it exists)
Look at the induced function $f_h$, which is a function from $\X \rightarrow \pmone$
The induced complexity of $f_h$ is $\ell$.
We need $g$ that operates on $\Z_\ell$ to get at the point that $h$ is not in $H_{\ell-1}$.
(and so for later - we will say $v$ is in some $H_\ell \setminus H_{\ell-1}$, so the definition of induced complexity needs to go through general functions $g$ - and not to be tied directly to $h$)}
\todo{state intuitively what this means}
\nir{not sure what to do with the above...}




%\outline{corollary: $F_k$ is composed only of $\ell$-set modular functions,
%for all $\ell \le k$, (i.e., different $f \in F$ can have different $\ell$-s)}


-----------------------------------------------------
\subsection{Stuff Moved From Sec 4.3}




modular:
--------
for $k=1$, the algorithm return $h$ which is modular
claim: setting $k=1$ is equivalent to choosing thresh-modular functions as hypothesis class
conclusion: algorithm works also for mmodular functions (and not just for all functions + $k$ complexity constraint)





subadditive:
------------
result: you get nothing out of choosing more complex subadditive functions
(modular is the "simplest" subadditive function)
let $H$=all set functions on reps of sizes between $k_1,k_2$
claim: thresh-modular functions $\equiv$ $H_1$
- "equiv" = algorithm with input $k=1$ returns an optimal $h$ that
behaves exactly like some thresh-modular function
(for general $k$, the algorithm returns a "wrapper" algorithm  that works on all rep sizes by lifting - this is essentially a little loop over $h_k$)
in the case of $k=1$,  

above is based on this result:
Take an $h \in H_k$ which is thresholding on a sub-additive set function. In particular, say $h(z) = \sign(g(z))$, and $g$ is sub-additive set function on $E$. Further, suppose $h(z)=1$ that is $g(z)\geq 0$, and $|z| = k$. Then for every $k'<k$ there exists a $z' \subseteq z$ such that $g(z') \geq 0$. In particular for every $h \in H_k$ and $k' <k$ there is a $h'\in H_{k'}$ such that $h$ is a lift of $H'$.


-----------------------------------------------

\outline{• fairness: when susceptibility correlates with some other attribute}


%=================================================================

% \paragraph{Tradeoff.}
% - if $k \le \ell^*$, then there's no tradeoff \\
% \outline{[result]: if $k \le \ell^*$, the empirical error = 0} \\

% - if $k> \ell^*$, there's a tradeoff \\
% \outline{[RESULT]: diminishing returns example}

% \paragraph{Knowing $\ell^*$ helps.}

% --- if $\ell^*< k_2$, then just set $k=\ell*$:
% \outline{[RESULT]: if $\ell^*< k_2$ then $k=\ell^*$ is the smallest $k$ that gives 0 empirical error}

% -- if $\ell*>k2$, set $k=k2$; otherwise set $k=\max\{\ell*,k1\}$ (or set  $k=\ell*$ and lift to $k1$ if $k1>\ell*$)
% \outline{11. corr: if $\ell*>k2$, then the optimal $h*$ is such that $h*'$ is $k2$-set modular}
% then the approximation error is minimized for an $h \in H_{k_2}$ which is not in $H_{k_2 - 1}$.




%------------------------------------------------------------




















%------------------------------------------------------------
%  Here, we ask following two questions; does    optimal  solution $h_T$ on empirical distribution $\widehat{D}$ (learned from samples $T$) an approximately optimal solution in terms of User's utility on true distribution $D$ (convergence); i.e. $\mathcal{U}(h_T) \geq \mathcal{U}(h) - \varepsilon $ (or $\mathcal{U}(h_T) \geq  \varepsilon \cdot  \mathcal{U}(h)  $ ) and second, how does local errors (wrong $h(z)$ due to uncertainty about the true distribution) affect the global performance.  
 
%\vineet{A possible approach for learning -- 1) Suppose we have the training set $T =\{(x_1, v(x_1)), (x_2, v(x_2)), \ldots, (x_n,v(x_n)\}$. 2) First we would create a training set for the user in the representation space. To this end let me call $h^*$ the optimal $h$ for the user. Also, let $D_{\Z}$ be the distribution induced by $D$ on the representation space $\Z$ (we can think of this as weighted normalization; will explain in detail during the meeting), and let us all call $\text{err}(h) = \mathbb{E}_{z \sim D_{\Z}}\{h(z) \neq h^{*}(z)\}$. c) Now this is the crucial part: Can we construct a $\tilde{h}$ using the above DP approach such that $\text{err}(h) = \mathbb{E}_{z \sim D_{\Z}}\{h(z) \neq h^{*}(z)\} \leq \epsilon$, where $\epsilon$ is dependent on the $n$ (no. of samples)? d) I think we might be able to; run the above DP algorithm on $T$ treating $\X$ as just $\{x_1, \ldots , x_n\}$ and $\Z$ as all possible representations of $\{x_1, \ldots, x_n\}$. Obviously $\tilde{h}$ would not be $h^*$ but we might be able to bound the error. Note that as $n \rightarrow \infty$, we can construct $\tilde{h} = h^*$ using the above DP. }
     %Fix $(h,\phi)$. Let $(z_{i}, h(z_{i}) )_{i=1}^{n}$ be $n$ representations obtained from i.i.d. samples $x_{i} \sim D$. Then can we learn $D_Z$ from these samples? If yes, we are interested in the finite time PAC bounds.
     %\paragraph{The learning question} 
     



==> proofs.tex <==
\section{Missing Proofs}

 \samePayoff* 
 \begin{proof}
The proof follows from the definition of best response. Let $z_1, z_2 \in \rep_h(x)$. Then since $\rep_h$ consists of only best response, we have either $h(z_1) = h(z_2) = 1$, or $h(z_1) = h(z_2) = -1$. Hence, $h(z_1) = v(x)$ if and only if $h(z_2) = v(x)$ for any $z_1, z_2 \in \phi_h(x)$.
\end{proof}

%\begin{proof}
%The proof follows from the fact that the  System's response can be decomposed into it's response to individual sampled items. Let $\phi_h$ and $\phi_{h}^{'} $ be two best responses such that $ h(\phi_{h}(x)) \neq h(\phi_{h}^{'}(x)) $  for some $x \in X$. Without loss of generality, let $h(\phi_h(x)) = 1$ and  $h(\phi_h^{'}(x)) = -1$. First let   $v(x) = -1$. In this case, as $\phi_{h}^{'}(x)$ is a best response we have that $h(z) = -1$ for all $z \in Z_x$. In particular, $h(\phi_{h}(x)) = -1$, a contradiction. On the other hand if $ v(x) = 1$ we have that there is at-least one $z \in Z_x$ (in particular, $z = \phi_{h}(x)$) such that $h(z) =1$ hence $\phi_{h}^{'}(x)$ is not a best response to $x$. A contradiction.      
%\end{proof}
\iffalse
\begin{proof}
The proof follows from the fact that the  System's response can be decomposed into it's response to individual sampled items. Let $\phi_h$ and $\phi_{h}^{'} $ be two best responses such that $ h(\phi_{h}(x)) \neq h(\phi_{h}^{'}(x)) $  for some $x \in X$. Without loss of generality, let $h(\phi_h(x)) = 1$ and  $h(\phi_h^{'}(x)) = -1$. First let   $v(x) = -1$. In this case, as $\phi_{h}^{'}(x)$ is a best response we have that $h(z) = -1$ for all $z \in Z_x$. In particular, $h(\phi_{h}(x)) = -1$; a contradiction. On the other hand if $ v(x) = 1$ we have that there is at least one $z \in Z_x$ (in particular, $z = \phi_{h}(x)$) such that $h(z) =1$ hence $\phi_{h}^{'}(x)$ is not a best response.      
\end{proof}
\fi
%\userPayoff*
\begin{proof}
We have  \begin{align*}
    \mathcal{U}(h) &= \sum_{x \sim D(X)}  \mathbbm{1}(h(\phi_h(x))= v(x))  \\& = \sum_{x \sim D(X)}  \sum_{z \in Z}  \cdot \mathbbm{1}(\phi_h(x)=z)   \cdot    \big ( \frac{h(z) \cdot v(x) +1}{2} \big ) \\
 & =    \frac{1}{2} \cdot \sum_{z \in Z}  \sum_{x| \phi_{h}(x) = z}  D(x) \cdot h(z) \cdot  v(x)  + \frac{1}{2} %   \\     &= 2 \cdot \mathbb{P}_{x \sim D } (h(\phi_{h}(x)) = v(x) ) -1 
%    & = \sum_{x \in X} \sum_{z \in N(x)} \mathbbm{1}(\phi_h(x)=z) \cdot  p_x \cdot  v(x) \cdot  h(z) 
\end{align*}
%\textcolor{red}{This result can be easily extended to randomized representation System strategy $\phi$ but as  there exists a deterministic $\phi$ for every optimal randomized $\phi$ hence we can restrict our attention to deterministic strategies of System WLOG}
\end{proof}
%\SVC*
\begin{proof}
By construction we have 
$$ h^{'}(\phi_{h^{'}}(x)) = h(\phi_{h}(\phi_{h^{'}}(x))) \text{ for some } h \in \mathcal{H}$$
Note that since $h$ is modular, any representation of $\phi_{h^{'}}(x)$ is also a representation of $x$. Also as $\phi_{h^{'}}(x)$ is a strategic representation of itself. Hence, we have 
\begin{align*} h^{'}(\phi_{h^{'}}(x)) = h(\phi_{h}(\phi_{h^{'}}(x))) &= \text{sign}(\langle \boldsymbol{u}, \phi_{h}(\phi_{h^{'}}(x)) \rangle ) \\ &= \text{sign}(\langle \boldsymbol{u}, \phi_{h}(x)\rangle ) \\ &= h(\phi_h(x)) = h^{'}(x)\end{align*}
\end{proof}

%\modular*
\begin{proof}
Let $h^{'} \in \mathcal{H}^{'}$ and, for contradiction assume that $h^{'} \notin \mathcal{J}$. Hence, there exists some $x$ and $x^{'} \subseteq x$ such that $h^{'}(x) = -1$ and $h^{'}(x^{'}) = +1$. Since $h^{'} \in \mathcal{H}^{'}$, we have $h^{'}(x^{'}) = h(\phi_{h}(x^{'})) = +1$ for some $h\in \mathcal{H}$. As the representation space consists of at most $k$ elements every representation of $x^{'}$ is a valid representation of $x$. Hence, we have $ +1 = h(\phi_{h}(x^{'})) = h(\phi_{h}(x)) = h^{'}(x) $, a contradiction. We have $\mathcal{H} \subseteq \mathcal{J}$. 

On the other hand, to show that $\mathcal{J} \subseteq \mathcal{H}^{'}$ it is enough to show that for every $h^{'} \in \mathcal{J}$  there is an  $h \in \mathcal{H}$ such that $h(\phi_{h}(x)) = h^{'}(x)$ for all $x$. In particular, for $h = h^{'}$ this condition is satisfied. 
\end{proof} 

\agnostic*
\begin{proof}
\textbf{CASE 1 (Strategic System):} Let $m = |Z_{x}|$ for every $x \in X$. Notice that if there is a $z$ such that $h(z)=1$ then it is a best response of the system. Write $z_{(1)}, z_{(2)} ... z_{(m)}$ such that $\phi_{h}(x)= z_{(i)}$ if $h(z_{(i)})=1$ and  $h(z_{(j)}) = -1 $ for all $j<i$. Next note that,
\begin{align*}
    \mathbb{P}(h(\phi_{h}(x)) =1) &= \mathbb{P}(\exists z \in Z_{x} \text{ such that } h(z)=1)  = \sum_{i=1}^{m} \mathbb{P}(z_{(i) }=1)\Pi_{j<i} \mathbb{P}(z_{(j) } =-1) \\
    & = \sum_{i=1}^{m} \alpha(1-\alpha)^{i-1} = \frac{\alpha (1 - (1-\alpha)^{m})}{\alpha} =1 - (1-\alpha)^{m}
    \intertext{Similarly, }
    \mathbb{P}(h(\phi_{h}(x)) = -1) &= \mathbb{P}(h(z) = -1 \text{ for all } z \in Z) =  (1-\alpha)^{m}.
\end{align*}
User's payoff is given by 
\begin{align*}
    \mathbb{P}_{x \sim X}[h(\phi_{h}(x)) = v(x)] &= \mathbb{P}(X^{+}) \mathbb{P}(h(\phi_{h}(x)) =1) + \mathbb{P}(X^{-}) \mathbb{P}(h(\phi_{h}(x)) =-1) \\
    & = \mathbb{P}(X^{+}) (1 - (1-\alpha)^{m}) + (1 - \mathbb{P}(X^{+}))  (1-\alpha)^{m}\\
    & = \mathbb{P}(X^{+}) + (1-\alpha)^{m} (1-2\cdot \mathbb{P}(X^{+})) 
\end{align*}
The payoff in above equation is  maximized  for $\alpha = 1$ when $\mathbb{P}(X^{+}) \geq 1/2$ and for $\alpha =0$ and when $\mathbb{P}(X^{+}) < 1/2$.

\textbf{CASE 2 (Benevolent System):} User's payoff is given as \begin{align*}
    \mathbb{P}_{x \sim X}[h(\phi_{h}(x)) = v(x)] &= \mathbb{P}( X^{+}) \cdot  \mathbb{P}(\exists z \text{ s.t. } h(z) = 1) + \mathbb{P}( X^{-})\mathbb{P}(\exists z \text{ s.t. } h(z) = -1) \\ 
    &= \mathbb{P}( X^{+}) (1 - (1-\alpha)^{m}) + (1-\mathbb{P}( X^{+}))(1-\alpha^{m}) \\ &= 1 - \alpha^{m} + \mathbb{P}(X^{+})(\alpha^{m} - (1-\alpha)^{m})
\end{align*}
When $\alpha=1 $ i.e. when $\mathbb{P}(X^{+}) \geq 1/2$,  User's payoff is given as  $\mathbb{P}(X^{+})$. On the other hand, it is  $\mathbb{P}(X^{-})$ when $\alpha=0$ i.e. $\mathbb{P}(X^{+}) < 1/2$. 

Note: In fact, in this case, User  can do even better by setting %$\alpha = \frac{1}{1+ (1/\mathbb{P}(X^{+}) -1)^{1/(m-1)}}$ 
$\alpha = \sqrt[m-1]{\mathbb{P} (X^{+})}$ for $m\geq 2$.  For instance, with $m=2$ we have, $\mathcal{U}(h_{agn})=1 - \mathbb{P}(X^{+})\mathbb{P}(X^{-}) \geq 3/4$. For $m=10$ we  have $\mathcal{U}(h_{agn}) \approx  0.9995$ close to \naive\ users payoff.   
\end{proof}

%\section{Additional results}
%\subsection{Learning Agnostic User's strategy} \ganesh{Use Hoeffding's inequality and claim that with probability at-least $1 - e^{-n\varepsilon^2}$ we have  $\mathbb{P}(X^{+}) \geq \frac{1}{n}\sum_{i=1}^{n} \mathbbm{1}(v(x_1) = 1) - \varepsilon$. Hence, expected payoff to the agnostic User when she learns her value function from data is given as $\frac{1-e^{-n\varepsilon^2}}{2}$ }


==> set_modular_hierarchy.tex <==
\section{Set-Modular Functions and its Hierarchy}
%Recall $E$ is the ground set of $q$ elements, $\mathfrak{P}(E)$ denotes the power set of $E$.
Let $Z_k \subset \mathfrak{P}(E)$ denote the set of subsets of $E$ of size equal to $k$. 
We have $Z_n = X \subseteq \mathfrak{P}(E)$, as the set of all possible item descriptions  and  $Z \subseteq  \mathfrak{P}(E)$ is the set of representation space. Throughout we assume that $Z = \cup_{k_1 \leq k\leq  k_2}Z_{k}$.



\begin{lemma}
\begin{enumerate}
    \item Let $h: Z \rightarrow \{-1,1\}$. Then there exists  $k \in [k_1,k_2]$ and  $\tilde{h}: Z_k \rightarrow \{-1,1\}$ such that for all $x$, $h(\phi_h(x)) = 1$ if there exists a $z\subset x$, $z \in Z_k$ such that $\tilde{h}(x) = 1$, and otherwise $h(\phi_h(x)) = -1$.
    \item Let $k \in [1, k_2]$, and $\tilde{h}: Z_k \rightarrow \{-1,1\}$. Then there is an $h: Z \rightarrow \{-1,1\}$ such that for all $x$, $h(\phi_h(x)) = 1$ if there exists a $z\subset x$ such that $\tilde{h}(z) = 1$, and otherwise $h(\phi_h(x)) = -1$. %\ganesh{I think it is $\tilde{h}(z)$ instead of $\tilde{h}(x)$ above.}
\end{enumerate}
\end{lemma}
\begin{proof}
Let $h: Z \rightarrow \{-1,1\}$, and $k = \max_{k' \in [k_1,k_2]} \{\text{there exists } z \text{ of size } k' \text{ such that } h(z) = 1 \text{ but for all } z'\subset z\ h(z') = -1\}$. Let $\tilde{h}: Z_k \rightarrow \{-1,1\}$ be as follows: for $z \in Z_k$, $\tilde{h}(z) = 1$ if there exists $z'\subseteq z$ such that $h(z) =1$ and otherwise it is $\tilde{h}(z) = -1$. From the construction of $\tilde{h}$ it follows that for all $x$, $h(\phi_h(x)) = 1$ if there exists a $z\subset x$, $z \in Z_k$ such that $\tilde{h}(x) = 1$, and otherwise $h(\phi_h(x)) = -1$.

Let $k \in [1, k_2]$, and $\tilde{h}: Z_k \rightarrow \{-1,1\}$. Define $h: Z \rightarrow \{-1,1\}$ as follows: a) If $k>k1$ then for $z\in Z$ and $|z| < k$, $h(z) = -1$, and for $z\in Z$ and $|z| >= k$, $h(z) = 1$ if there exists $z' \subseteq z$ and $z' \in Z_k$ such that $\tilde{h}(z') = 1$. From the construction. it follows that, for all $x$, $h(\phi_h(x)) = 1$ if there exists a $z\subset x$, $z \in Z_k$ such that $\tilde{h}(x) = 1$, and otherwise $h(\phi_h(x)) = -1$.
\end{proof}

\begin{definition} 
A map $g:X \rightarrow \{-1,1\}$ is $k$-set modular if there exist a map $h: Z_{k} \rightarrow \{-1,1\}$ such that $g(x) = 1$ if there exists $z \in Z_k$ and $z \subseteq x$ such that $h(z) = 1$ and otherwise $-1$.
\end{definition}

\begin{observation}
Any function $g:X \rightarrow \{-1,1\}$ is $n$-set modular. 
\end{observation}

From Observation \toref\ we have that the value function $v: X \rightarrow \{-1,1\}$ of a user is $n$-set modular.

\begin{lemma}
For every $k \in [2,n]$ there exists $g:X \rightarrow \{-1,1\}$ such that $g$ is $k$-set modular but not $k'$-set modular for $k'<k$.
\end{lemma}
\begin{proof}
Arbitrarily choose a $z \in Z_k$, and let $S_z = \{z' \in Z_k \mid |z' \cap z| = k-1\}$. Let $h: Z_k \rightarrow \{-1,1\}$ be such that $h(z)=1$ and for all $z' \neq z$, $h(z) = -1$. Now let $g: X \rightarrow \{-1,1\}$ be such that for all $x$ such that $z \subset x$ $g(x) = 1$, and otherwise $g(x) = -1$. It is clear that $g$ is $k$ set-modular, as $g(x) = 1$ if and only if there exists a $z \subset x$, $z \in Z_k$ such that $h(z')=1$. Now we show that $g$ is not $k-1$ set-modular.

Say $g$ is $k'$ set modular for some $k'< k$. Then there exists a $\tilde{h}: Z_{k'} \rightarrow \{-1,1\}$ such that $g(x) = 1$ if and only if there exists a $z'\subset x$ and $z'\in Z_{k'}$ such that $\tilde{h}(z') = 1$. Choose an $x \in X$ such that $z \subset x$ and hence, $g(x) =1$. This implies there exists a $z' \subset x$ and $z'\in Z_{k'}$ such that $\tilde{h}(z')=1$. Since $q> n$, and $k' < k$ we have an $x \in X$ such that $z' \subset x$ but $z \not\subset x$. Since  $z \not\subset x$ we have $g(x) = -1$ but as $\tilde{h}(z') =1$ we have $g(x) = 1$. This gives a contradiction.

\end{proof}

Let $k^* = \min_{k \in [1,n]} \{v \text{ is } k\text{-set modular}\}$.

\begin{lemma}
\begin{enumerate}
    \item If $k^* \leq k_2$ then there exists $h: Z \rightarrow \{-1,1\}$ such that $h(\phi_h(x)) = v(x)$ for all $x\in X$.
    \item If $k^* > k_2$ and $\mathcal{H} = \{h: Z \rightarrow \{-1,1\} \}$ then $h^* = \arg \min_{h\in \mathcal{H}}\{E_{x \sim D}\mathbbm{1}\{h(\phi_h(x)) =  v(x)\}\}$ is such that there does not exists a $k< k_2$ and $h_{k}:Z_{k} \rightarrow \{-1,1\}$ satisfying the following: $h^*(\phi_{h^*}(x)) = 1$ if there exists a $z\subset x$ and $z \in Z_{k}$ such that $h_{k}(z) =1$ and otherwise $h^*(\phi_{h^*}(x)) = -1$. 
\end{enumerate}
\end{lemma}



\begin{lemma}
Let $g:X \rightarrow \{-1,1\}$ be $k$-set-modular. Then there exists $a_+ > 0$ and $a_{-}<0$ and $w:Z_k \rightarrow \{a_-,a_+\}$ such that $g(x) = \text{sign}(\sum_{z \subseteq x, z\in Z_k} w(z))$.
\end{lemma}


==> todo.tex <==
\nir{can/should $v$ be stochastic? if yes, then in what way, and what is known to who about its randomness?}
\vineet{a) If $v$ is made stochastic then the utility of both the user and the system would have in their respective expressions the distribution over which $v$ is defined. b) I think the motivation to make $v$ stochastic is that in real world $v$ is never exact and stochasticity in $v$ is a way to incorporate noisy behaviour; in some sense having $v(x) = 1$ with prob 0.9 says that 9/10 times the user would choose $x$, c) In this sense the stochastic nature of user is known neither to the user or the system?}
Here, expectation is taken over randomness in the ``state of the world" (i.e.  $D$) and randomness in  learning algorithm, if any \footnote{For now we assume that $h$ is deterministic. It is not clear if a randomized $h$ provide strictly larger  payoff to User. }.
